DuoLoRA : Cycle-consistent and Rank-disentangled Content-Style Personalization

We tackle the challenge of jointly personalizing content and style from a few examples. A promising approach is to train separate Low-Rank Adapters (LoRA) and merge them effectively, preserving both content and style. Existing methods, such as ZipLoRA, treat content and style as independent entities, merging them by learning masks in LoRA's output dimensions. However, content and style are intertwined, not independent. To address this, we propose DuoLoRA, a content-style personalization framework featuring three key components: (i) rank-dimension mask learning, (ii) effective merging via layer priors, and (iii) Constyle loss, which leverages cycle-consistency in the merging process. First, we introduce ZipRank, which performs content-style merging within the rank dimension, offering adaptive rank flexibility and significantly reducing the number of learnable parameters. Additionally, we incorporate SDXL layer priors to apply implicit rank constraints informed by each layer's content-style bias and adaptive merger initialization, enhancing the integration of content and style. To further refine the merging process, we introduce Constyle loss, which leverages the cycle-consistency between content and style. Our experimental results demonstrate that DuoLoRA outperforms state-of-the-art content-style merging methods across multiple benchmarks.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Personalizing text-to-image diffusion models~\cite{ruiz2023dreambooth,sohn2023styledrop,chang2023muse} has recently attracted significant interest due to their broad range of applications. Personalizing both content and style from limited examples, however, is particularly challenging. Earlier approaches in neural style transfer required extensive training data to blend content and style effectively. To address this data limitation, parameter-efficient fine-tuning (PEFT) methods like Low-Rank Adapters (LoRA)~\cite{hu2021lora} have become popular, as learning low-rank adapters can sufficiently capture unique characteristics. As a result, content-style personalization can be reframed as a LoRA merging task, where individually trained LoRAs are combined to achieve efficient content-style blending. Recent methods, such as ZipLoRA~\cite{shah2025ziplora}, merge content and style by learning masks over the LoRA output dimensions, assuming that content and style are independent concepts.

\begin{figure}
    \centering
        \centering
        \includegraphics[width=0.5\textwidth]{figures/problem.png} % second figure itself
        \caption{Content and style personalization : LoRA blending }
        \label{fig:problem}  
        \vspace{-0.2cm}
 \end{figure}
 
However, using the same rank for both content and style LoRAs may not be optimal, as content and style may have different representational requirements and thus benefit from varying ranks. Adaptive rank flexibility could enable more effective LoRA blending. To achieve this, we propose learning masks in the rank dimension rather than in the output dimension, which allows for adaptive rank adjustment while significantly reducing the number of learnable parameters.

To implement rank adaptability across the layers of the diffusion UNet, we analyze the SDXL model architecture~\cite{basu2024mechanistic, frenkel2024implicit}. We observe that the early layers of the UNet, characterized by lower receptive fields, contribute more to content generation; therefore, content mergers should have a higher rank in these layers than style mergers. In contrast, later layers with higher receptive fields play a larger role in style generation, and the rank constraint should be reversed~\cite{basu2024mechanistic, frenkel2024implicit}. For layer-wise rank-adaptive merging, we enforce these rank constraints during content-style merging. This rank constraint is reformulated as a nuclear norm minimization problem under an $l1$ sparsity constraint, improving content-style blending with fewer learnable parameters.

While these layer-wise rank constraints establish a rank hierarchy, they don’t guarantee a consistent margin between ranks, which may vary across layers and potentially lead to trivial solutions. For instance, if content is given a much higher rank than style in early layers, style might be overshadowed, leading to content-biased blending. To address this, we introduce a feedback mechanism to maintain an optimal margin between ranks by using cycle-consistency across content and style. This approach, inspired by StyleGAN’s~\cite{karras2019style} method of treating content and style as two domains and optimizing their blending through domain translation with a minimized reconstruction loss, allows for balanced content-style merging. Unlike ZipLoRA~\cite{karras2019style}, which treats content and style as independent concepts, our cycle-consistency loss accounts for their intertwined nature, resulting in improved content-style blending.

In summary, the contributions of this paper are as follows:

\begin{itemize} 
    \item We address content-style personalization as a LoRA merging problem, where we propose learning masks in the rank dimension instead of the output dimension, allowing for adaptive rank flexibility with significantly fewer learnable parameters. 
    \item We analyze the SDXL architecture’s layer prior information, finding that early layers (receptive field <32) primarily contribute to content generation, while later layers (receptive field =32) focus on style generation. Based on these insights, we introduce explicit rank constraints through nuclear norm minimization under a sparsity constraint to improve merging. 
    \item We introduce layer-adaptive control of rank difference margins by incorporating a cycle-consistency loss across content and style, and we validate this approach across various benchmarks. 
\end{itemize}

==> sec/2.0_preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminary}

\textbf{Low-Rank Adaptation (LoRA): }
In LoRA~\cite{hu2021lora}, we fine-tune neural networks by approximating weight updates using low-rank matrices. Specifically, the weight update matrix $\Delta W$ is parameterized as:
\[
\Delta W = A B,
\]
where: \[
A \in \mathbb{R}^{d_{\text{out}} \times r}, \quad B \in \mathbb{R}^{r \times d_{\text{in}}},
\] and $r$ is the rank of the approximation.
\newline
\textbf{Best Rank-$r$ Approximation: }
By the Eckart-Young-Mirsky Theorem~\cite{golub1987generalization}, the best rank-$r$ approximation of $X$ (in terms of minimizing the Frobenius norm of the error) is:
\[
X_r = U_r \Sigma_r V_r^\top,
\]
with:
\[
U_r \in \mathbb{R}^{d_{\text{out}} \times r} \quad \text{(first $r$ columns of $U$)},
\]
\[
\Sigma_r = \operatorname{diag}(\sigma_1, \sigma_2, \dots, \sigma_r),
\]
\[
V_r \in \mathbb{R}^{d_{\text{in}} \times r} \quad \text{(first $r$ columns of $V$)}.
\]
The minimal approximation error is:
\[
E_{\min} = \| X - X_r \|_F = \left( \sum_{i = r+1}^{p} \sigma_i^2 \right)^{1/2}.
\]

==> sec/2.5_theoretical_analysis.tex <==
\section{Theoretical analysis}
\label{sec:theoretical_analysis}

\begin{lemma}
\label{Lemma:lemma_1}
Let \( m_c \in \mathbb{R}^{m \times n} \) be a matrix representing the content and \( m_s \in \mathbb{R}^{m \times n} \) be a matrix representing the style. The problem of minimizing the \( L_1 \)-norm of \( m_c \) subject to a rank constraint on \( m_c \) can be written as:
\[
\min \|m_c\|_1 \quad \text{subject to} \quad \text{rank}(m_c) > \text{rank}(m_s)
\]
This problem is non-convex due to the rank constraint. A convex relaxation can be achieved by approximating the rank of a matrix using the nuclear norm \( \| \cdot \|_* \), which is the sum of the singular values of the matrix. Thus, the original problem can be relaxed to:
\[
\min \|m_c\|_1 \quad \text{subject to} \quad \|m_c\|_* > \|m_s\|_*
\]
where \( \|m_c\|_* \) denotes the nuclear norm of \( m_c \), and \( \|m_s\|_* \) is the nuclear norm of \( m_s \).

This relaxed problem can be approached via a Lagrangian penalty formulation:
\[
\mathcal{L}(m_c, \lambda) = \|m_c\|_1 + \lambda \max(0, \|m_s\|_* - \|m_c\|_*)
\]
for some penalty parameter \( \lambda \geq 0 \), which enforces the constraint \( \|m_c\|_* > \|m_s\|_* \) in the limit as \( \lambda \to \infty \).
\end{lemma}

\begin{proof}
    Proof is provided in the supplementary material.
\end{proof}

% \begin{definition} {Lipschitz Regularity :}
% A function $f: \mathbb{R}^n \to \mathbb{R}^m$ is Lipschitz continuous if there exists a constant $L \geq 0$ such that for all $x_1, x_2 \in \mathbb{R}^n$,
% \[
% \| f(x_1) - f(x_2) \| \leq L \| x_1 - x_2 \|
% \]
% The smallest such $L$ is called the Lipschitz constant of $f$. Lipschitz regularity ensures that the rate of change of the function is controlled, and thus the function behaves in a stable manner.
% \end{definition}

% \begin{definition}{Cycle consistency :}
% This implies that applying a forward transformation followed by an inverse transformation approximately returns the original input. Let $T_1: \mathbb{R}^n \to \mathbb{R}^m$ and $T_2: \mathbb{R}^m \to \mathbb{R}^n$ be two transformations (e.g., content and style transformations), then cycle consistency demands that for all $x \in \mathbb{R}^n$ and $y \in \mathbb{R}^m$:
% \[
% T_2(T_1(x)) \approx x \quad \text{and} \quad T_1(T_2(y)) \approx y
% \]
% Mathematically, this can be written as:
% \[
% \| T_2(T_1(x)) - x \| \leq \epsilon_1 \quad \text{and} \quad \| T_1(T_2(y)) - y \| \leq \epsilon_2
% \]
% for small tolerances $\epsilon_1, \epsilon_2 > 0$. 
% \end{definition}


% \begin{Proposition}
% \label{proposition:proposition_1}
%     Cycle consistency provides Lipschitz regularity in merging.
% \end{Proposition}
% \begin{proof}
% The proof is provided in the supplementary material.

% % If both $T_1$ and $T_2$ are Lipschitz continuous with Lipschitz constants $L_1$ and $L_2$, respectively, then combining them in a cycle should preserve Lipschitz regularity.

% % \begin{itemize}
% %     \item{Forward Transformation:}
% % Consider $T_1: \mathbb{R}^n \to \mathbb{R}^m$. To ensure Lipschitz regularity, we have:
% % \[
% % \| T_1(x_1) - T_1(x_2) \| \leq L_1 \| x_1 - x_2 \|
% % \]
% % \[
% % \| T_2(x_1) - T_2(x_2) \| \leq L_2 \| x_1 - x_2 \|
% % \]
% %     \item {Backward Transformation (Cycle Consistency)}
% % The reverse transformation $T_2$ should satisfy:
% % \[
% % \| T_2(T_1(x_1)) - T_2(T_1(x_2)) \| \leq L_2 \| T_1(x_1) - T_1(x_2) \|
% % \]
% % \end{itemize}
% % Substituting the Lipschitz bound for $T_1$, we get:
% % \[
% % \| T_2(T_1(x_1)) - T_2(T_1(x_2)) \| \leq L_2 L_1 \| x_1 - x_2 \|
% % \]
% % Thus, the composite function $T_2 \circ T_1$ is also Lipschitz continuous, with Lipschitz constant $L_1 L_2$.

% Cycle consistency naturally imposes constraints on the transformations $T_1$ and $T_2$. 
% To enforce Lipschitz regularity through cycle consistency, we introduce a cycle-consistency loss:
% \[
% L_{\text{cycle}} = \| T_2(T_1(x)) - x \|^2
% \]
% By minimizing this loss during training, we encourage the forward and backward transformations to be consistent, thereby implicitly regularizing the Lipschitz constants of the merged transformations. If the cycle-consistency loss is small, it implies that the transformations are stable, i.e., small changes in the input result in small changes in the output, thereby enforcing Lipschitz continuity.


% Diffusion models are not inherently Lipschitz continuous. However, recent research in score-based diffusion models~\cite{chen2022sampling, chen2023improved}, particularly those incorporating spectral normalization, promotes Lipschitz continuity, especially within their score functions. Cycle consistency further encourages Lipschitz regularity by stabilizing domain transformations, ensuring that small changes in the input produce proportionate changes in the output. This regularity enhances both the stability and quality of style transfer, reducing the risk of artifacts and preserving content structure even after transformation across domains, as demonstrated empirically in Fig.~\ref{fig:qual_2}.

% \end{proof}

\begin{definition}{Rank Dimension Masking : }
We apply a mask to the rank dimension by defining a diagonal mask matrix $M_r \in \mathbb{R}^{r \times r}$ with entries $m_{ii} \in \{0, 1\}$. The rank-masked approximation is:
\[
\Delta W_{\text{rank}} = A M_r B = U_r M_r \Sigma_r V_r^\top.
\]
Let $S$ denote the set of indices $i$ where $m_{ii} = 1$, and $s = |S|$ is the number of active rank components.
\end{definition}


\begin{definition}{Output Dimension Masking: }
We apply a mask to the output dimension by defining a diagonal mask matrix $M_{\text{out}} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{out}}}$ with entries $n_{ii} \in \{0, 1\}$. The output-masked approximation is:
\[
\Delta W_{\text{out}} = M_{\text{out}} A B = M_{\text{out}} U_r \Sigma_r V_r^\top.
\]
Let $d_s = \sum_{i=1}^{d_{\text{out}}} n_{ii}$ be the number of active output units.
\end{definition}

\begin{theorem} In LoRA merging, under the same parameter budget, the approximation error resulting from rank dimension masking is less than or equal to that from output dimension masking. Formally,
\[
E_{\text{rank}} \leq E_{\text{out}},
\]
where:
\[
E_{\text{rank}} = \| X - \Delta W_{\text{rank}} \|_F
\]
is the approximation error using rank dimension masking, and
\[
E_{\text{out}} = \| X - \Delta W_{\text{out}} \|_F
\]
is the approximation error using output dimension masking.
\label{theroem:output_rank_merging}
\end{theorem}

\begin{proof}
Proof is provided in the supplementary material.
\end{proof}

\begin{figure*}
    \centering
        \centering
        \includegraphics[width=0.95\textwidth]{figures/method_2.png} % second figure itself
        \caption{Cycle consistency merging}
        \label{fig:cycle_consistency}   
 \end{figure*}
% To compare the two masking strategies fairly, we ensure that both use the same number of parameters.
% Parameter Count for Rank Dimension Masking, 
% \[
% P_{\text{rank}} = s (d_{\text{out}} + d_{\text{in}}).
% \]
% Parameter Count for Output Dimension Masking is,
% \[
% P_{\text{out}} = d_s \times r + r \times d_{\text{in}} = r (d_s + d_{\text{in}}).
% \]

% Now, Setting Equal Parameter Budgets,
% Set $P_{\text{rank}} = P_{\text{out}}$:
% \[
% s (d_{\text{out}} + d_{\text{in}}) = r (d_s + d_{\text{in}}).
% \]
% Assuming $d_{\text{out}} = d_{\text{in}} = d$ for simplicity:
% \[
% s (2d) = r (d_s + d).
% \]
% Solving for $s$:
% \[
% s = \frac{r (d_s + d)}{2d}.
% \]


% Next, we compare the Approximation Errors.

% Since we retain the $s$ largest singular values to minimize the error, the approximation error for Rank Dimension Masking is:
% \[
% E_{\text{rank}} = \left( \sum_{i = s+1}^{p} \sigma_i^2 \right)^{1/2}.
% \]

% The exact computation of Output Dimension Masking error ($E_{\text{out}}$) is complex due to the loss of orthogonality in $U_r$ caused by masking. However, we can establish a lower bound.

% The total energy (sum of squares) in $U_r$ is:
% \[
% \| U_r \|_F^2 = \operatorname{trace}(U_r^\top U_r) = r.
% \]
% where each row of $U_r$ contributes equally on average to this total energy.

% The fraction of rows masked out (i.e., energy removed by masking) is:
% \[
% f = \frac{d - d_s}{d}.
% \]
% Therefore, the approximate fraction of energy removed is $f$.

% \textbf{Lower Bound on Approximation Error:}

% Next, we get the lower bound on Approximation Error, i.e., the loss in the approximation due to output dimension masking is at least:
% \[
% E_{\text{out}}^2 \geq f \sum_{i=1}^{r} \sigma_i^2 + \sum_{i = r+1}^{p} \sigma_i^2.
% \]

% The first term $f \sum_{i=1}^{r} \sigma_i^2$ represents the loss from masking out a fraction $f$ of the energy from the top $r$ singular values. The second term $\sum_{i = r+1}^{p} \sigma_i^2$ accounts for the singular values beyond rank $r$.


% Now, Relating $s$ and $f$, from the parameter equality:
% \[
% s = \frac{r (d_s + d)}{2d} = \frac{r}{2} \left( 1 + \frac{d_s}{d} \right).
% \]
% Since $d_s = d (1 - f)$:
% \[
% \begin{align*}
% s &= \frac{r}{2} \left( 1 + \frac{d_s}{d} \right) \\
%   &= \frac{r}{2} \left( 1 + (1 - f) \right) \\
%   &= \frac{r}{2} (2 - f) \\
%   &= r \left( 1 - \frac{f}{2} \right).
% \end{align*}
% \]
% Thus,
% \[
% \frac{s}{r} = 1 - \frac{f}{2}.
% \]

% We observe, in Rank Dimension Masking :
% The approximation error comes from the discarded smaller singular values (indices $i > s$).
% Since $s = r \left( 1 - \frac{f}{2} \right)$, we discard the smallest $r - s = r \left( \frac{f}{2} \right)$ singular values among the top $r$.
% \[
% E_{\text{rank}}^2 = \sum_{i=s+1}^{p} \sigma_i^2 = \sum_{i=r\left(1 - \frac{f}{2}\right)+1}^{p} \sigma_i^2.
% \]

% In Output Dimension Masking:
% The error includes a loss from the largest singular values, scaled by $f$, because masking affects all components equally.
% \[
% E_{\text{out}}^2 \geq f \sum_{i=1}^{r} \sigma_i^2 + \sum_{i=r+1}^{p} \sigma_i^2.
% \]


% \textbf{Mathematical Comparison:}

% Total Energy of Top $r$ Singular Values

% \[
% q = \sum_{i=1}^{r} \sigma_i^2.
% \]

% Sum of Discarded Singular Values in Rank Masking:

% \[
% q' = \sum_{i = s+1}^{r} \sigma_i^2 = q - \sum_{i=1}^{s} \sigma_i^2.
% \]

% Relation between $f$ and $\frac{s}{r}$:

% \[
% f = 2 \left( 1 - \frac{s}{r} \right).
% \]

% \textbf{Expressing $E_{\text{rank}}^2$ and $E_{\text{out}}^2$ in terms of $q$ and $q'$:}

% Rank Dimension Masking Error:

% \[
% E_{\text{rank}}^2 = q' + \sum_{i = r+1}^{p} \sigma_i^2.
% \]

% Output Dimension Masking Error Lower Bound:

% \[
% E_{\text{out}}^2 \geq f q + \sum_{i = r+1}^{p} \sigma_i^2.
% \]

% Since $q' = q - \sum_{i=1}^{s} \sigma_i^2$ and $s = r \left( 1 - \frac{f}{2} \right)$, we have:

% \[
% \begin{align*}
% q' &= q - \sum_{i=1}^{s} \sigma_i^2 \\
%    &\leq q - s \left( \frac{\sigma_r^2}{r} \cdot r \right) \quad (\text{since } \sigma_i \geq \sigma_r) \\
%    &= q - s \sigma_r^2 \\
%    &= q - r \left( 1 - \frac{f}{2} \right) \sigma_r^2.
% \end{align*}
% \]

% Therefore,

% \[
% E_{\text{rank}}^2 \leq q - r \left( 1 - \frac{f}{2} \right) \sigma_r^2 + \sum_{i = r+1}^{p} \sigma_i^2.
% \]

% \textbf{Comparing with $E_{\text{out}}^2$:}

% \[
% E_{\text{out}}^2 \geq f q + \sum_{i = r+1}^{p} \sigma_i^2.
% \]

% Since $f = 2 \left( 1 - \frac{s}{r} \right)$, we have:

% \[
% E_{\text{out}}^2 \geq 2 \left( 1 - \frac{s}{r} \right) q + \sum_{i = r+1}^{p} \sigma_i^2.
% \]

% Therefore, the difference between $E_{\text{out}}^2$ and $E_{\text{rank}}^2$ is:

% \[
% E_{\text{out}}^2 - E_{\text{rank}}^2 \geq \left[ 2 \left( 1 - \frac{s}{r} \right) q - \left( q - r \left( 1 - \frac{f}{2} \right) \sigma_r^2 \right) \right]\\
% = \left( 1 - \frac{s}{r} \right) \left( q + r \sigma_r^2 \right).
% \]

% Since $q \geq r \sigma_r^2$, the difference is non-negative, implying:

% \[
% E_{\text{rank}}^2 \leq E_{\text{out}}^2.
% \]

